DOTA: A Large-scale Dataset for Object Detection in Aerial Images

Object detection is an important and challenging problem in computer vision. Although the past decade has witnessed major advances in object detection in natural scenes, such successes have been slow to aerial imagery, not only because of the huge variation in the scale, orientation and shape of the object instances on the earth's surface, but also due to the scarcity of well-annotated datasets of objects in aerial scenes. To advance object detection research in Earth Vision, also known as Earth Observation and Remote Sensing, we introduce a large-scale Dataset for Object deTection in Aerial images (DOTA). To this end, we collect $2806$ aerial images from different sensors and platforms. Each image is of the size about 4000-by-4000 pixels and contains objects exhibiting a wide variety of scales, orientations, and shapes. These DOTA images are then annotated by experts in aerial image interpretation using $15$ common object categories. The fully annotated DOTA images contains $188,282$ instances, each of which is labeled by an arbitrary (8 d.o.f.) quadrilateral To build a baseline for object detection in Earth Vision, we evaluate state-of-the-art object detection algorithms on DOTA. Experiments demonstrate that DOTA well represents real Earth Vision applications and are quite challenging.

==> pixelsizepicutre.tex <==
\begin{figure*}
\begin{center}
%\subfigure[]{

% \includegraphics[width=0.18\textwidth]{pixelsize/baseball-diamond.eps}%
% \hspace{0.0000in}%
% \includegraphics[width=0.18\textwidth]{pixelsize/basketball-court.eps}
%\hspace{0in}
\subfigure {
	\includegraphics[width=0.23\textwidth]{pixelsize/bridge-eps-converted-to.pdf}%
	\hspace{0in}%
	\includegraphics[width=0.23\textwidth]{pixelsize/ground-track-field-eps-converted-to.pdf}%
	\hspace{0in}%
	\includegraphics[width=0.23\textwidth]{pixelsize/harbor-eps-converted-to.pdf}%
	\hspace{0in}%
	\includegraphics[width=0.23\textwidth]{pixelsize/helicopter-eps-converted-to.pdf}%
}
\subfigure{
	\includegraphics[width=0.23\textwidth]{pixelsize/small-vehicle-eps-converted-to.pdf}
	\hspace{0in}
	\includegraphics[width=0.23\textwidth]{pixelsize/large-vehicle-eps-converted-to.pdf}
	\hspace{0in}
	\includegraphics[width=0.23\textwidth]{pixelsize/ship-eps-converted-to.pdf}
	\hspace{0in}
	\includegraphics[width=0.23\textwidth]{pixelsize/plane-eps-converted-to.pdf}
}


% \hspace{0in}
% \includegraphics[width=0.23\textwidth]{pixelsize/soccer-ball-field-eps-converted-to.pdf}
% \hspace{0in}
% \includegraphics[width=0.26\textwidth]{pixelsize/storage-tank-eps-converted-to.pdf}
% \hspace{0in}
% \includegraphics[width=0.18\textwidth]{pixelsize/tennis-court-eps-converted-to.pdf}
% \hspace{0in}
% \includegraphics[width=0.18\textwidth]{pixelsize/swimming-pool-eps-converted-to.pdf}
% \hspace{0in}
% \includegraphics[width=0.18\textwidth]{pixelsize/turntable-eps-converted-to.pdf}

%}

\end{center}
    \caption{Pixel size of selected categories}
\label{fig:pixel-size}
\end{figure*}

==> trash.tex <==
\begin{table}[htb!]
\scriptsize
\centering
\begin{tabular}{c|c|c|c|c||c}
\hline
           & YOLOv2\cite{yolo9000}           & R-FCN\cite{R-FCN}          & FR-H\cite{FasterR-CNN}           & SSD\cite{SSD} & FR-O\cite{FasterR-CNN}           \\ \hline
\textit{Plane}              & 76.9           & 79.33          & 80.32 &  44.74   & 79.09          \\
\textit{BD}   & 33.87          & 44.26          & 77.55 &   11.21  & 69.12          \\
\textit{Bridge}             & 22.73          & 36.58 & 32.86          &   6.22  & 17.17          \\
\textit{GTF} & 34.88          & 53.53          & 68.13 &  6.91  & 63.49          \\
\textit{SV}      & 38.73          & 39.38          & 53.66 &  2  & 34.2           \\
\textit{LV}      & 32.02          & 34.15          & 52.49 &  10.24   & 37.16          \\
\textit{Ship}               & 52.37 & 47.29          & 50.04          &  11.34   & 36.2           \\
\textit{TC}       & 61.65          & 45.66          & 90.41 &  15.59   & 89.19          \\
\textit{BC}   & 48.54          & 47.74          & 75.05 &  12.56   & 69.6           \\
\textit{ST}       & 33.91          & 65.84 & 59.59          &  17.94   & 58.96          \\
\textit{SBF}  & 29.27          & 37.92          & 57    &  14.73   & 49.4           \\
\textit{RA}         & 36.83          & 44.23          & 49.81          &  4.55   & 52.52 \\
\textit{Harbor}             & 36.44          & 47.23          & 61.69 &  4.55   & 46.69          \\
\textit{SP}      & 38.26          & 50.64          & 56.46 &  0.53   & 44.8           \\
\textit{HC}         & 11.61          & 34.9           & 41.85          &  1.01   & 46.3  \\ \hline
\textit{\textbf{Avg.}}               & 39.2           & 47.24          & 60.46 &  10.94   & 52.93          \\ \hline
\end{tabular}
\vspace{-2mm}
\caption{Numerical results of baseline models (AP). The short names for categories are defined as: {\em BD--Baseball diamond, GTF--Ground field track, SV--Small vehicle,  LV--Large vehicle, TC--Tennis court, BC--Basketball court, SC--Storage tank, SBF--Soccer-ball field, RA--Roundabout, SP--Swimming pool, and  HC--Helicopter}. FR-H means \textbf{F}aster \textbf{R}-CNN~\cite{FasterR-CNN} trained on \textbf{H}orizontal bounding boxes. FR-O means \textbf{F}aster \textbf{R}-CNN~\cite{FasterR-CNN} trained on \textbf{O}riented bounding boxes.}
\label{numericalresults}
\end{table}
